Learning Local Volt/Var Controllers Towards Efficient Network Operation with Stability Guarantees

This paper considers the problem of voltage regulation in distribution networks. The primary motivation is to keep voltages within preassigned operating limits by commanding the reactive power output of distributed energy resources (DERs) deployed in the grid. We develop a framework for developing local Volt/Var control that comprises two main steps. In the first, by exploiting historical data and for each DER, we learn a function representing the desirable equilibrium points for the power network. These points approximate solutions of an Optimal Power Flow (OPF) problem. In the second, we propose a control scheme for steering the network towards these favorable configurations. Theoretical conditions are derived to formally guarantee the stability of the developed control scheme, and numerical simulations illustrate the effectiveness of the proposed approach.

==> stylesV2.tex <==
% function definitions
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\range}{range}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\nullspace}{null}
\DeclareMathOperator{\pr}{Pr}
\DeclareMathOperator{\Beta}{B}
\DeclareMathOperator{\diag}{dg}
\DeclareMathOperator{\bdiag}{bdg}
\DeclareMathOperator{\trace}{Tr}
\DeclareMathOperator{\vectorize}{vec}
\DeclareMathOperator{\real}{Re}
\DeclareMathOperator{\imag}{Im}
\DeclareMathOperator{\maximum}{max}
\DeclareMathOperator{\minimum}{min}
\DeclareMathOperator{\signum}{sign}
\DeclareMathOperator{\MLE}{MLE}
\DeclareMathOperator{\subjectto}{s.to}
\DeclareMathOperator{\prox}{prox}
\DeclareMathOperator{\dimension}{dim}
\DeclareMathOperator*{\find}{find}
%\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
%\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}

% theorem environments
\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}

% colored text
\newcommand\cmr[1]{\textcolor{red}{#1}}
\newcommand\cmb[1]{\textcolor{blue}{#1}}
\newcommand\cmg[1]{\textcolor{green}{#1}}

% % all definitions go in the order
% - numbers
% - small Latin letters
% - capital Latin letters
% - small Greek letters
% - capital Greek letters


%%%% BOLD
\newcommand \bzero{\mathbf{0}}
\newcommand \bone{\mathbf{1}}
\newcommand \ba{\mathbf{a}}
\newcommand \bb{\mathbf{b}}
\newcommand \bc{\mathbf{c}}
\newcommand \bd{\mathbf{d}}
\newcommand \be{\mathbf{e}}
\newcommand \bef{\mathbf{f}} % exception since \bf is taken
\newcommand \bg{\mathbf{g}}
\newcommand \bh{\mathbf{h}}
\newcommand \bi{\mathbf{i}}
\newcommand \bj{\mathbf{j}}
\newcommand \bk{\mathbf{k}}
\newcommand \bdell{\boldsymbol{\ell}} % \bell is already taken
\newcommand \bm{\mathbf{m}}
\newcommand \bn{\mathbf{n}}
\newcommand \bo{\mathbf{o}}
\newcommand \bp{\mathbf{p}}
\newcommand \bq{\mathbf{q}}
\newcommand \br{\mathbf{r}}
\newcommand \bs{\mathbf{s}}
\newcommand \bt{\mathbf{t}}
\newcommand \bu{\mathbf{u}}
\newcommand \bv{\mathbf{v}}
\newcommand \bw{\mathbf{w}}
\newcommand \bx{\mathbf{x}}
\newcommand \by{\mathbf{y}}
\newcommand \bz{\mathbf{z}}
\newcommand \bA{\mathbf{A}}
\newcommand \bB{\mathbf{B}}
\newcommand \bC{\mathbf{C}}
\newcommand \bD{\mathbf{D}}
\newcommand \bE{\mathbf{E}}
\newcommand \bF{\mathbf{F}}
\newcommand \bG{\mathbf{G}}
\newcommand \bH{\mathbf{H}}
\newcommand \bI{\mathbf{I}}
\newcommand \bJ{\mathbf{J}}
\newcommand \bK{\mathbf{K}}
\newcommand \bL{\mathbf{L}}
\newcommand \bM{\mathbf{M}}
\newcommand \bN{\mathbf{N}}
\newcommand \bO{\mathbf{O}}
\newcommand \bP{\mathbf{P}}
\newcommand \bQ{\mathbf{Q}}
\newcommand \bR{\mathbf{R}}
\newcommand \bS{\mathbf{S}}
\newcommand \bT{\mathbf{T}}
\newcommand \bU{\mathbf{U}}
\newcommand \bV{\mathbf{V}}
\newcommand \bW{\mathbf{W}}
\newcommand \bX{\mathbf{X}}
\newcommand \bY{\mathbf{Y}}
\newcommand \bZ{\mathbf{Z}}
\newcommand \balpha{\boldsymbol{\alpha}}
\newcommand \bbeta{\boldsymbol{\beta}}
\newcommand \bgamma{\boldsymbol{\gamma}}
\newcommand \bdelta{\boldsymbol{\delta}}
\newcommand \bepsilon{\boldsymbol{\epsilon}}
\newcommand \bzeta{\boldsymbol{\zeta}}
\newcommand \bdeta{\boldsymbol{\eta}} %% bdeta to differentiate from beta
\newcommand \btheta{\boldsymbol{\theta}}
\newcommand \biota{\boldsymbol{\iota}}
\newcommand \bkappa{\boldsymbol{\kappa}}
\newcommand \blambda{\boldsymbol{\lambda}}
\newcommand \bmu{\boldsymbol{\mu}}
\newcommand \bnu{\boldsymbol{\nu}}
\newcommand \bxi{\boldsymbol{\xi}}
\newcommand \bpi{\boldsymbol{\pi}}
\newcommand \brho{\boldsymbol{\rho}}
\newcommand \bsigma{\boldsymbol{\sigma}}
\newcommand \btau{\boldsymbol{\tau}}
\newcommand \bupsilon{\boldsymbol{\upsilon}}
\newcommand \bphi{\boldsymbol{\phi}}
\newcommand \bchi{\boldsymbol{\chi}}
\newcommand \bpsi{\boldsymbol{\psi}}
\newcommand \bomega{\boldsymbol{\omega}}
\newcommand \bGamma{\mathbf{\Gamma}}
\newcommand \bDelta{\mathbf{\Delta}}
\newcommand \bTheta{\mathbf{\Theta}}
\newcommand \bvarTheta{\boldsymbol{\varTheta}}
\newcommand \bLambda{\mathbf{\Lambda}}
\newcommand \bXi{\mathbf{\Xi}}
\newcommand \bPi{\mathbf{\Pi}}
\newcommand \bSigma{\mathbf{\Sigma}}
\newcommand \bPhi{\mathbf{\Phi}}
\newcommand \bPsi{\mathbf{\Psi}}
\newcommand \bOmega{\mathbf{\Omega}}


%%%% TILDE
\newcommand \tda{\tilde{a}}
\newcommand \tdb{\tilde{b}}
\newcommand \tdc{\tilde{c}}
\newcommand \tdd{\tilde{d}}
\newcommand \tde{\tilde{e}}
\newcommand \tdf{\tilde{f}}
\newcommand \tdh{\tilde{h}}
\newcommand \tdi{\tilde{i}}
\newcommand \tdj{\tilde{j}}
\newcommand \tdk{\tilde{k}}
\newcommand \tdell{\tilde{\ell}}
\newcommand \tdm{\tilde{m}}
\newcommand \tdn{\tilde{n}}
\newcommand \tdo{\tilde{o}}
\newcommand \tdp{\tilde{p}}
\newcommand \tdq{\tilde{q}}
\newcommand \tdr{\tilde{r}}
\newcommand \tds{\tilde{s}}
\newcommand \tdt{\tilde{t}}
\newcommand \tdu{\tilde{u}}
\newcommand \tdv{\tilde{v}}
\newcommand \tdw{\tilde{w}}
\newcommand \tdx{\tilde{x}}
\newcommand \tdy{\tilde{y}}
\newcommand \tdz{\tilde{z}}
\newcommand \tdA{\tilde{A}}
\newcommand \tdB{\tilde{B}}
\newcommand \tdC{\tilde{C}}
\newcommand \tdD{\tilde{D}}
\newcommand \tdE{\tilde{E}}
\newcommand \tdF{\tilde{F}}
\newcommand \tdG{\tilde{G}}
\newcommand \tdH{\tilde{H}}
\newcommand \tdI{\tilde{I}}
\newcommand \tdK{\tilde{K}}
\newcommand \tdL{\tilde{L}}
\newcommand \tdM{\tilde{M}}
\newcommand \tdN{\tilde{N}}
\newcommand \tdO{\tilde{O}}
\newcommand \tdP{\tilde{P}}
\newcommand \tdQ{\tilde{Q}}
\newcommand \tdR{\tilde{R}}
\newcommand \tdS{\tilde{S}}
\newcommand \tdT{\tilde{T}}
\newcommand \tdU{\tilde{U}}
\newcommand \tdV{\tilde{V}}
\newcommand \tdW{\tilde{W}}
\newcommand \tdX{\tilde{X}}
\newcommand \tdY{\tilde{Y}}
\newcommand \tdZ{\tilde{Z}}
\newcommand \tdalpha{\tilde{\alpha}}
\newcommand \tdbeta{\tilde{\beta}}
\newcommand \tdgamma{\tilde{\gamma}}
\newcommand \tddelta{\tilde{\delta}}
\newcommand \tdepsilon{\tilde{\epsilon}}
\newcommand \tdzeta{\tilde{\zeta}}
\newcommand \tdeta{\tilde{\eta}}
\newcommand \tdtheta{\tilde{\theta}}
\newcommand \tdiota{\tilde{\iota}}
\newcommand \tdkappa{\tilde{\kappa}}
\newcommand \tdlambda{\tilde{\lambda}}
\newcommand \tdmu{\tilde{\mu}}
\newcommand \tdnu{\tilde{\nu}}
\newcommand \tdxi{\tilde{\xi}}
\newcommand \tdpi{\tilde{\pi}}
\newcommand \tdrho{\tilde{\rho}}
\newcommand \tdsigma{\tilde{\sigma}}
\newcommand \tdtau{\tilde{\tau}}
\newcommand \tdupsilon{\tilde{\upsilon}}
\newcommand \tdphi{\tilde{\phi}}
\newcommand \tdchi{\tilde{\chi}}
\newcommand \tdpsi{\tilde{\psi}}
\newcommand \tdomega{\tilde{\omega}}
\newcommand \tdGamma{\tilde{\Gamma}}
\newcommand \tdDelta{\tilde{\Delta}}
\newcommand \tdTheta{\tilde{\Theta}}
\newcommand \tdLambda{\tilde{\Lambda}}
\newcommand \tdXi{\tilde{\Xi}}
\newcommand \tdPi{\tilde{\Pi}}
\newcommand \tdSigma{\tilde{\Sigma}}
\newcommand \tdPhi{\tilde{\Phi}}
\newcommand \tdPsi{\tilde{\Psi}}
\newcommand \tdOmega{\tilde{\Omega}}

%%%% HAT
\newcommand \hta{\hat{a}}
\newcommand \htb{\hat{b}}
\newcommand \htc{\hat{c}}
\newcommand \htd{\hat{d}}
\newcommand \hte{\hat{e}}
\newcommand \htf{\hat{f}}
\newcommand \hth{\hat{h}}
\newcommand \hti{\hat{i}}
\newcommand \htj{\hat{j}}
\newcommand \htk{\hat{k}}
\newcommand \htell{\hat{\ell}}
\newcommand \htm{\hat{m}}
\newcommand \htn{\hat{n}}
\newcommand \hto{\hat{o}}
\newcommand \htp{\hat{p}}
\newcommand \htq{\hat{q}}
\newcommand \htr{\hat{r}}
\newcommand \hts{\hat{s}}
\newcommand \htt{\hat{t}}
\newcommand \htu{\hat{u}}
\newcommand \htv{\hat{v}}
\newcommand \htw{\hat{w}}
\newcommand \htx{\hat{x}}
\newcommand \hty{\hat{y}}
\newcommand \htz{\hat{z}}
\newcommand \htA{\hat{A}}
\newcommand \htB{\hat{B}}
\newcommand \htC{\hat{C}}
\newcommand \htD{\hat{D}}
\newcommand \htE{\hat{E}}
\newcommand \htF{\hat{F}}
\newcommand \htG{\hat{G}}
\newcommand \htH{\hat{H}}
\newcommand \htI{\hat{I}}
\newcommand \htK{\hat{K}}
\newcommand \htL{\hat{L}}
\newcommand \htM{\hat{M}}
\newcommand \htN{\hat{N}}
\newcommand \htO{\hat{O}}
\newcommand \htP{\hat{P}}
\newcommand \htQ{\hat{Q}}
\newcommand \htR{\hat{R}}
\newcommand \htS{\hat{S}}
\newcommand \htT{\hat{T}}
\newcommand \htU{\hat{U}}
\newcommand \htV{\hat{V}}
\newcommand \htW{\hat{W}}
\newcommand \htX{\hat{X}}
\newcommand \htY{\hat{Y}}
\newcommand \htZ{\hat{Z}}
\newcommand \htalpha{\hat{\alpha}}
\newcommand \htbeta{\hat{\beta}}
\newcommand \htgamma{\hat{\gamma}}
\newcommand \htdelta{\hat{\delta}}
\newcommand \htepsilon{\hat{\epsilon}}
\newcommand \htzeta{\hat{\zeta}}
\newcommand \htdeta{\hat{\eta}} %% bdeta to differentiate from beta
\newcommand \httheta{\hat{\theta}}
\newcommand \htiota{\hat{\iota}}
\newcommand \htkappa{\hat{\kappa}}
\newcommand \htlambda{\hat{\lambda}}
\newcommand \htmu{\hat{\mu}}
\newcommand \htnu{\hat{\nu}}
\newcommand \htxi{\hat{\xi}}
\newcommand \htpi{\hat{\pi}}
\newcommand \htrho{\hat{\rho}}
\newcommand \htsigma{\hat{\sigma}}
\newcommand \httau{\hat{\tau}}
\newcommand \htupsilon{\hat{\upsilon}}
\newcommand \htphi{\hat{\phi}}
\newcommand \htchi{\hat{\chi}}
\newcommand \htpsi{\hat{\psi}}
\newcommand \htomega{\hat{\omega}}
\newcommand \htGamma{\hat{\Gamma}}
\newcommand \htDelta{\hat{\Delta}}
\newcommand \htTheta{\hat{\Theta}}
\newcommand \htLambda{\hat{\Lambda}}
\newcommand \htXi{\hat{\Xi}}
\newcommand \htPi{\hat{\Pi}}
\newcommand \htSigma{\hat{\Sigma}}
\newcommand \htPhi{\hat{\Phi}}
\newcommand \htPsi{\hat{\Psi}}
\newcommand \htOmega{\hat{\Omega}}

%%%% CHECK
\newcommand \cha{\check{a}}
\newcommand \chb{\check{b}}
\newcommand \chc{\check{c}}
\newcommand \chd{\check{d}}
\newcommand \che{\check{e}}
\newcommand \chf{\check{f}}
\newcommand \chh{\check{h}}
\newcommand \chj{\check{j}}
\newcommand \chk{\check{k}}
\newcommand \chell{\check{\ell}}
\newcommand \chm{\check{m}}
\newcommand \chn{\check{n}}
\newcommand \cho{\check{o}}
\newcommand \chp{\check{p}}
\newcommand \chq{\check{q}}
\newcommand \chr{\check{r}}
\newcommand \chs{\check{s}}
\newcommand \cht{\check{t}}
\newcommand \chu{\check{u}}
\newcommand \chv{\check{v}}
\newcommand \chw{\check{w}}
\newcommand \chx{\check{x}}
\newcommand \chy{\check{y}}
\newcommand \chz{\check{z}}
\newcommand \chA{\check{A}}
\newcommand \chB{\check{B}}
\newcommand \chC{\check{C}}
\newcommand \chD{\check{D}}
\newcommand \chE{\check{E}}
\newcommand \chF{\check{F}}
\newcommand \chG{\check{G}}
\newcommand \chH{\check{H}}
\newcommand \chI{\check{I}}
\newcommand \chK{\check{K}}
\newcommand \chL{\check{L}}
\newcommand \chM{\check{M}}
\newcommand \chN{\check{N}}
\newcommand \chO{\check{O}}
\newcommand \chP{\check{P}}
\newcommand \chQ{\check{Q}}
\newcommand \chR{\check{R}}
\newcommand \chS{\check{S}}
\newcommand \chT{\check{T}}
\newcommand \chU{\check{U}}
\newcommand \chV{\check{V}}
\newcommand \chW{\check{W}}
\newcommand \chX{\check{X}}
\newcommand \chY{\check{Y}}
\newcommand \chZ{\check{Z}}
\newcommand \chalpha{\check{\alpha}}
\newcommand \chbeta{\check{\beta}}
\newcommand \chgamma{\check{\gamma}}
\newcommand \chdelta{\check{\delta}}
\newcommand \chepsilon{\check{\epsilon}}
\newcommand \chzeta{\check{\zeta}}
\newcommand \chdeta{\check{\eta}} %% bdeta to differentiate from beta
\newcommand \chtheta{\check{\theta}}
\newcommand \chiota{\check{\iota}}
\newcommand \chkappa{\check{\kappa}}
\newcommand \chlambda{\check{\lambda}}
\newcommand \chmu{\check{\mu}}
\newcommand \chnu{\check{\nu}}
\newcommand \chxi{\check{\xi}}
\newcommand \chpi{\check{\pi}}
\newcommand \chrho{\check{\rho}}
\newcommand \chsigma{\check{\sigma}}
\newcommand \chtau{\check{\tau}}
\newcommand \chupsilon{\check{\upsilon}}
\newcommand \chphi{\check{\phi}}
\newcommand \chchi{\check{\chi}}
\newcommand \chpsi{\check{\psi}}
\newcommand \chomega{\check{\omega}}
\newcommand \chGamma{\check{\Gamma}}
\newcommand \chDelta{\check{\Delta}}
\newcommand \chTheta{\check{\Theta}}
\newcommand \chLambda{\check{\Lambda}}
\newcommand \chXi{\check{\Xi}}
\newcommand \chPi{\check{\Pi}}
\newcommand \chSigma{\check{\Sigma}}
\newcommand \chPhi{\check{\Phi}}
\newcommand \chPsi{\check{\Psi}}
\newcommand \chOmega{\check{\Omega}}


%%%% MATHCAL
\newcommand \mcA{\mathcal{A}}
\newcommand \mcB{\mathcal{B}}
\newcommand \mcC{\mathcal{C}}
\newcommand \mcD{\mathcal{D}}
\newcommand \mcE{\mathcal{E}}
\newcommand \mcF{\mathcal{F}}
\newcommand \mcG{\mathcal{G}}
\newcommand \mcH{\mathcal{H}}
\newcommand \mcI{\mathcal{I}}
\newcommand \mcK{\mathcal{K}}
\newcommand \mcL{\mathcal{L}}
\newcommand \mcM{\mathcal{M}}
\newcommand \mcN{\mathcal{N}}
\newcommand \mcO{\mathcal{O}}
\newcommand \mcP{\mathcal{P}}
\newcommand \mcQ{\mathcal{Q}}
\newcommand \mcR{\mathcal{R}}
\newcommand \mcS{\mathcal{S}}
\newcommand \mcT{\mathcal{T}}
\newcommand \mcU{\mathcal{U}}
\newcommand \mcV{\mathcal{V}}
\newcommand \mcW{\mathcal{W}}
\newcommand \mcX{\mathcal{X}}
\newcommand \mcY{\mathcal{Y}}
\newcommand \mcZ{\mathcal{Z}}

%%%% BAR-MATHCAL (complements of sets)
\newcommand \bmcA{\bar{\mathcal{A}}}
\newcommand \bmcB{\bar{\mathcal{B}}}
\newcommand \bmcC{\bar{\mathcal{C}}}
\newcommand \bmcD{\bar{\mathcal{D}}}
\newcommand \bmcE{\bar{\mathcal{E}}}
\newcommand \bmcF{\bar{\mathcal{F}}}
\newcommand \bmcG{\bar{\mathcal{G}}}
\newcommand \bmcH{\bar{\mathcal{H}}}
\newcommand \bmcI{\bar{\mathcal{I}}}
\newcommand \bmcJ{\bar{\mathcal{J}}}
\newcommand \bmcK{\bar{\mathcal{K}}}
\newcommand \bmcL{\bar{\mathcal{L}}}
\newcommand \bmcM{\bar{\mathcal{M}}}
\newcommand \bmcN{\bar{\mathcal{N}}}
\newcommand \bmcO{\bar{\mathcal{O}}}
\newcommand \bmcP{\bar{\mathcal{P}}}
\newcommand \bmcQ{\bar{\mathcal{Q}}}
\newcommand \bmcR{\bar{\mathcal{R}}}
\newcommand \bmcS{\bar{\mathcal{S}}}
\newcommand \bmcT{\bar{\mathcal{T}}}
\newcommand \bmcU{\bar{\mathcal{U}}}
\newcommand \bmcV{\bar{\mathcal{V}}}
\newcommand \bmcW{\bar{\mathcal{W}}}
\newcommand \bmcX{\bar{\mathcal{X}}}
\newcommand \bmcY{\bar{\mathcal{Y}}}
\newcommand \bmcZ{\bar{\mathcal{Z}}}

%%%% TILDE-MATHCAL
\newcommand \tmcA{\tilde{\mathcal{A}}}
\newcommand \tmcB{\tilde{\mathcal{B}}}
\newcommand \tmcC{\tilde{\mathcal{C}}}
\newcommand \tmcD{\tilde{\mathcal{D}}}
\newcommand \tmcE{\tilde{\mathcal{E}}}
\newcommand \tmcF{\tilde{\mathcal{F}}}
\newcommand \tmcG{\tilde{\mathcal{G}}}
\newcommand \tmcH{\tilde{\mathcal{H}}}
\newcommand \tmcI{\tilde{\mathcal{I}}}
\newcommand \tmcJ{\tilde{\mathcal{J}}}
\newcommand \tmcK{\tilde{\mathcal{K}}}
\newcommand \tmcL{\tilde{\mathcal{L}}}
\newcommand \tmcM{\tilde{\mathcal{M}}}
\newcommand \tmcN{\tilde{\mathcal{N}}}
\newcommand \tmcO{\tilde{\mathcal{O}}}
\newcommand \tmcP{\tilde{\mathcal{P}}}
\newcommand \tmcQ{\tilde{\mathcal{Q}}}
\newcommand \tmcR{\tilde{\mathcal{R}}}
\newcommand \tmcS{\tilde{\mathcal{S}}}
\newcommand \tmcT{\tilde{\mathcal{T}}}
\newcommand \tmcU{\tilde{\mathcal{U}}}
\newcommand \tmcV{\tilde{\mathcal{V}}}
\newcommand \tmcW{\tilde{\mathcal{W}}}
\newcommand \tmcX{\tilde{\mathcal{X}}}
\newcommand \tmcY{\tilde{\mathcal{Y}}}
\newcommand \tmcZ{\tilde{\mathcal{Z}}}


%%%% TILDE-BOLD
\newcommand \tba{\tilde{\mathbf{a}}}
\newcommand \tbb{\tilde{\mathbf{b}}}
\newcommand \tbc{\tilde{\mathbf{c}}}
\newcommand \tbd{\tilde{\mathbf{d}}}
\newcommand \tbe{\tilde{\mathbf{e}}}
\newcommand \tbf{\tilde{\mathbf{f}}}
\newcommand \tbh{\tilde{\mathbf{h}}}
\newcommand \tbi{\tilde{\mathbf{i}}}
\newcommand \tbj{\tilde{\mathbf{j}}}
\newcommand \tbk{\tilde{\mathbf{k}}}
\newcommand \tbell{\tilde{\mathbf{\ell}}}
\newcommand \tbm{\tilde{\mathbf{m}}}
\newcommand \tbn{\tilde{\mathbf{n}}}
\newcommand \tbo{\tilde{\mathbf{o}}}
\newcommand \tbp{\tilde{\mathbf{p}}}
\newcommand \tbq{\tilde{\mathbf{q}}}
\newcommand \tbr{\tilde{\mathbf{r}}}
\newcommand \tbs{\tilde{\mathbf{s}}}
\newcommand \tbt{\tilde{\mathbf{t}}}
\newcommand \tbu{\tilde{\mathbf{u}}}
\newcommand \tbv{\tilde{\mathbf{v}}}
\newcommand \tbw{\tilde{\mathbf{w}}}
\newcommand \tbx{\tilde{\mathbf{x}}}
\newcommand \tby{\tilde{\mathbf{y}}}
\newcommand \tbz{\tilde{\mathbf{z}}}
\newcommand \tbA{\tilde{\mathbf{A}}}
\newcommand \tbB{\tilde{\mathbf{B}}}
\newcommand \tbC{\tilde{\mathbf{C}}}
\newcommand \tbD{\tilde{\mathbf{D}}}
\newcommand \tbE{\tilde{\mathbf{E}}}
\newcommand \tbF{\tilde{\mathbf{F}}}
\newcommand \tbG{\tilde{\mathbf{G}}}
\newcommand \tbH{\tilde{\mathbf{H}}}
\newcommand \tbI{\tilde{\mathbf{I}}}
\newcommand \tbJ{\tilde{\mathbf{J}}}
\newcommand \tbK{\tilde{\mathbf{K}}}
\newcommand \tbL{\tilde{\mathbf{L}}}
\newcommand \tbM{\tilde{\mathbf{M}}}
\newcommand \tbN{\tilde{\mathbf{N}}}
\newcommand \tbO{\tilde{\mathbf{O}}}
\newcommand \tbP{\tilde{\mathbf{P}}}
\newcommand \tbQ{\tilde{\mathbf{Q}}}
\newcommand \tbR{\tilde{\mathbf{R}}}
\newcommand \tbS{\tilde{\mathbf{S}}}
\newcommand \tbT{\tilde{\mathbf{T}}}
\newcommand \tbU{\tilde{\mathbf{U}}}
\newcommand \tbV{\tilde{\mathbf{V}}}
\newcommand \tbW{\tilde{\mathbf{W}}}
\newcommand \tbX{\tilde{\mathbf{X}}}
\newcommand \tbY{\tilde{\mathbf{Y}}}
\newcommand \tbZ{\tilde{\mathbf{Z}}}
\newcommand \tbalpha{\tilde{\boldsymbol{\alpha}}}
\newcommand \tbbeta{\tilde{\boldsymbol{\beta}}}
\newcommand \tbgamma{\tilde{\boldsymbol{\gamma}}}
\newcommand \tbdelta{\tilde{\boldsymbol{\delta}}}
\newcommand \tbepsilon{\tilde{\boldsymbol{\epsilon}}}
\newcommand \tbzeta{\tilde{\boldsymbol{\zeta}}}
\newcommand \tbeta{\tilde{\boldsymbol{\eta}}}
\newcommand \tbtheta{\tilde{\boldsymbol{\theta}}}
\newcommand \tbiota{\tilde{\boldsymbol{\iota}}}
\newcommand \tbkappa{\tilde{\boldsymbol{\kappa}}}
\newcommand \tblambda{\tilde{\boldsymbol{\lambda}}}
\newcommand \tbmu{\tilde{\boldsymbol{\mu}}}
\newcommand \tbnu{\tilde{\boldsymbol{\nu}}}
\newcommand \tbxi{\tilde{\boldsymbol{\xi}}}
\newcommand \tbpi{\tilde{\boldsymbol{\pi}}}
\newcommand \tbrho{\tilde{\boldsymbol{\rho}}}
\newcommand \tbsigma{\tilde{\boldsymbol{\sigma}}}
\newcommand \tbtau{\tilde{\boldsymbol{\tau}}}
\newcommand \tbupsilon{\tilde{\boldsymbol{\upsilon}}}
\newcommand \tbphi{\tilde{\boldsymbol{\phi}}}
\newcommand \tbchi{\tilde{\boldsymbol{\chi}}}
\newcommand \tbpsi{\tilde{\boldsymbol{\psi}}}
\newcommand \tbomega{\tilde{\boldsymbol{\omega}}}
\newcommand \tbGamma{\tilde{\mathbf{\Gamma}}}
\newcommand \tbDelta{\tilde{\mathbf{\Delta}}}
\newcommand \tbTheta{\tilde{\mathbf{\Theta}}}
\newcommand \tbLambda{\tilde{\mathbf{\Lambda}}}
\newcommand \tbXi{\tilde{\mathbf{\Xi}}}
\newcommand \tbPi{\tilde{\mathbf{\Pi}}}
\newcommand \tbSigma{\tilde{\mathbf{\Sigma}}}
\newcommand \tbPhi{\tilde{\mathbf{\Phi}}}
\newcommand \tbPsi{\tilde{\mathbf{\Psi}}}
\newcommand \tbOmega{\tilde{\mathbf{\Omega}}}

%%%% CHECK-BOLD
\newcommand \cba{\check{\mathbf{a}}}
\newcommand \cbb{\check{\mathbf{b}}}
\newcommand \cbc{\check{\mathbf{c}}}
\newcommand \cbd{\check{\mathbf{d}}}
\newcommand \cbe{\check{\mathbf{e}}}
\newcommand \cbf{\check{\mathbf{f}}}
\newcommand \cbh{\check{\mathbf{h}}}
\newcommand \cbi{\check{\mathbf{i}}}
\newcommand \cbj{\check{\mathbf{j}}}
\newcommand \cbk{\check{\mathbf{k}}}
\newcommand \cbell{\check{\mathbf{\ell}}}
\newcommand \cbm{\check{\mathbf{m}}}
\newcommand \cbn{\check{\mathbf{n}}}
\newcommand \cbo{\check{\mathbf{o}}}
\newcommand \cbp{\check{\mathbf{p}}}
\newcommand \cbq{\check{\mathbf{q}}}
\newcommand \cbr{\check{\mathbf{r}}}
\newcommand \cbs{\check{\mathbf{s}}}
\newcommand \cbt{\check{\mathbf{t}}}
\newcommand \cbu{\check{\mathbf{u}}}
\newcommand \cbv{\check{\mathbf{v}}}
\newcommand \cbw{\check{\mathbf{w}}}
\newcommand \cbx{\check{\mathbf{x}}}
\newcommand \cby{\check{\mathbf{y}}}
\newcommand \cbz{\check{\mathbf{z}}}
\newcommand \cbA{\check{\mathbf{A}}}
\newcommand \cbB{\check{\mathbf{B}}}
\newcommand \cbC{\check{\mathbf{C}}}
\newcommand \cbD{\check{\mathbf{D}}}
\newcommand \cbE{\check{\mathbf{E}}}
\newcommand \cbF{\check{\mathbf{F}}}
\newcommand \cbG{\check{\mathbf{G}}}
\newcommand \cbH{\check{\mathbf{H}}}
\newcommand \cbI{\check{\mathbf{I}}}
\newcommand \cbK{\check{\mathbf{K}}}
\newcommand \cbL{\check{\mathbf{L}}}
\newcommand \cbM{\check{\mathbf{M}}}
\newcommand \cbN{\check{\mathbf{N}}}
\newcommand \cbO{\check{\mathbf{O}}}
\newcommand \cbP{\check{\mathbf{P}}}
\newcommand \cbQ{\check{\mathbf{Q}}}
\newcommand \cbR{\check{\mathbf{R}}}
\newcommand \cbS{\check{\mathbf{S}}}
\newcommand \cbT{\check{\mathbf{T}}}
\newcommand \cbU{\check{\mathbf{U}}}
\newcommand \cbV{\check{\mathbf{V}}}
\newcommand \cbW{\check{\mathbf{W}}}
\newcommand \cbX{\check{\mathbf{X}}}
\newcommand \cbY{\check{\mathbf{Y}}}
\newcommand \cbZ{\check{\mathbf{Z}}}
\newcommand \cbalpha{\check{\boldsymbol{\alpha}}}
\newcommand \cbbeta{\check{\boldsymbol{\beta}}}
\newcommand \cbgamma{\check{\boldsymbol{\gamma}}}
\newcommand \cbdelta{\check{\boldsymbol{\delta}}}
\newcommand \cbepsilon{\check{\boldsymbol{\epsilon}}}
\newcommand \cbzeta{\check{\boldsymbol{\zeta}}}
\newcommand \cbeta{\check{\boldsymbol{\eta}}}
\newcommand \cbtheta{\check{\boldsymbol{\theta}}}
\newcommand \cbiota{\check{\boldsymbol{\iota}}}
\newcommand \cbkappa{\check{\boldsymbol{\kappa}}}
\newcommand \cblambda{\check{\boldsymbol{\lambda}}}
\newcommand \cbmu{\check{\boldsymbol{\mu}}}
\newcommand \cbnu{\check{\boldsymbol{\nu}}}
\newcommand \cbxi{\check{\boldsymbol{\xi}}}
\newcommand \cbpi{\check{\boldsymbol{\pi}}}
\newcommand \cbrho{\check{\boldsymbol{\rho}}}
\newcommand \cbsigma{\check{\boldsymbol{\sigma}}}
\newcommand \cbtau{\check{\boldsymbol{\tau}}}
\newcommand \cbupsilon{\check{\boldsymbol{\upsilon}}}
\newcommand \cbphi{\check{\boldsymbol{\phi}}}
\newcommand \cbchi{\check{\boldsymbol{\chi}}}
\newcommand \cbpsi{\check{\boldsymbol{\psi}}}
\newcommand \cbomega{\check{\boldsymbol{\omega}}}
\newcommand \cbGamma{\check{\mathbf{\Gamma}}}
\newcommand \cbDelta{\check{\mathbf{\Delta}}}
\newcommand \cbTheta{\check{\mathbf{\Theta}}}
\newcommand \cbLambda{\check{\mathbf{\Lambda}}}
\newcommand \cbXi{\check{\mathbf{\Xi}}}
\newcommand \cbPi{\check{\mathbf{\Pi}}}
\newcommand \cbSigma{\check{\mathbf{\Sigma}}}
\newcommand \cbPhi{\check{\mathbf{\Phi}}}
\newcommand \cbPsi{\check{\mathbf{\Psi}}}
\newcommand \cbOmega{\check{\mathbf{\Omega}}}

%% HAT-BOLD
\newcommand \hba{\hat{\mathbf{a}}}
\newcommand \hbb{\hat{\mathbf{b}}}
\newcommand \hbc{\hat{\mathbf{c}}}
\newcommand \hbd{\hat{\mathbf{d}}}
\newcommand \hbe{\hat{\mathbf{e}}}
\newcommand \hbf{\hat{\mathbf{f}}}
\newcommand \hbh{\hat{\mathbf{h}}}
\newcommand \hbi{\hat{\mathbf{i}}}
\newcommand \hbj{\hat{\mathbf{j}}}
\newcommand \hbk{\hat{\mathbf{k}}}
\newcommand \hbell{\hat{\mathbf{\ell}}}
\newcommand \hbm{\hat{\mathbf{m}}}
\newcommand \hbn{\hat{\mathbf{n}}}
\newcommand \hbo{\hat{\mathbf{o}}}
\newcommand \hbp{\hat{\mathbf{p}}}
\newcommand \hbq{\hat{\mathbf{q}}}
\newcommand \hbr{\hat{\mathbf{r}}}
\newcommand \hbs{\hat{\mathbf{s}}}
\newcommand \hbt{\hat{\mathbf{t}}}
\newcommand \hbu{\hat{\mathbf{u}}}
\newcommand \hbv{\hat{\mathbf{v}}}
\newcommand \hbw{\hat{\mathbf{w}}}
\newcommand \hbx{\hat{\mathbf{x}}}
\newcommand \hby{\hat{\mathbf{y}}}
\newcommand \hbz{\hat{\mathbf{z}}}
\newcommand \hbA{\hat{\mathbf{A}}}
\newcommand \hbB{\hat{\mathbf{B}}}
\newcommand \hbC{\hat{\mathbf{C}}}
\newcommand \hbD{\hat{\mathbf{D}}}
\newcommand \hbE{\hat{\mathbf{E}}}
\newcommand \hbF{\hat{\mathbf{F}}}
\newcommand \hbG{\hat{\mathbf{G}}}
\newcommand \hbH{\hat{\mathbf{H}}}
\newcommand \hbI{\hat{\mathbf{I}}}
\newcommand \hbJ{\hat{\mathbf{J}}}
\newcommand \hbK{\hat{\mathbf{K}}}
\newcommand \hbL{\hat{\mathbf{L}}}
\newcommand \hbM{\hat{\mathbf{M}}}
\newcommand \hbN{\hat{\mathbf{N}}}
\newcommand \hbO{\hat{\mathbf{O}}}
\newcommand \hbP{\hat{\mathbf{P}}}
\newcommand \hbQ{\hat{\mathbf{Q}}}
\newcommand \hbR{\hat{\mathbf{R}}}
\newcommand \hbS{\hat{\mathbf{S}}}
\newcommand \hbT{\hat{\mathbf{T}}}
\newcommand \hbU{\hat{\mathbf{U}}}
\newcommand \hbV{\hat{\mathbf{V}}}
\newcommand \hbW{\hat{\mathbf{W}}}
\newcommand \hbX{\hat{\mathbf{X}}}
\newcommand \hbY{\hat{\mathbf{Y}}}
\newcommand \hbZ{\hat{\mathbf{Z}}}
\newcommand \hbalpha{\hat{\boldsymbol{\alpha}}}
\newcommand \hbbeta{\hat{\boldsymbol{\beta}}}
\newcommand \hbgamma{\hat{\boldsymbol{\gamma}}}
\newcommand \hbdelta{\hat{\boldsymbol{\delta}}}
\newcommand \hbepsilon{\hat{\boldsymbol{\epsilon}}}
\newcommand \hbzeta{\hat{\boldsymbol{\zeta}}}
\newcommand \hbeta{\hat{\boldsymbol{\eta}}}
\newcommand \hbtheta{\hat{\boldsymbol{\theta}}}
\newcommand \hbiota{\hat{\boldsymbol{\iota}}}
\newcommand \hbkappa{\hat{\boldsymbol{\kappa}}}
\newcommand \hblambda{\hat{\boldsymbol{\lambda}}}
\newcommand \hbmu{\hat{\boldsymbol{\mu}}}
\newcommand \hbnu{\hat{\boldsymbol{\nu}}}
\newcommand \hbxi{\hat{\boldsymbol{\xi}}}
\newcommand \hbpi{\hat{\boldsymbol{\pi}}}
\newcommand \hbrho{\hat{\boldsymbol{\rho}}}
\newcommand \hbsigma{\hat{\boldsymbol{\sigma}}}
\newcommand \hbtau{\hat{\boldsymbol{\tau}}}
\newcommand \hbupsilon{\hat{\boldsymbol{\upsilon}}}
\newcommand \hbphi{\hat{\boldsymbol{\phi}}}
\newcommand \hbchi{\hat{\boldsymbol{\chi}}}
\newcommand \hbpsi{\hat{\boldsymbol{\psi}}}
\newcommand \hbomega{\hat{\boldsymbol{\omega}}}
\newcommand \hbGamma{\hat{\mathbf{\Gamma}}}
\newcommand \hbDelta{\hat{\mathbf{\Delta}}}
\newcommand \hbTheta{\hat{\mathbf{\Theta}}}
\newcommand \hbLambda{\hat{\mathbf{\Lambda}}}
\newcommand \hbXi{\hat{\mathbf{\Xi}}}
\newcommand \hbPi{\hat{\mathbf{\Pi}}}
\newcommand \hbSigma{\hat{\mathbf{\Sigma}}}
\newcommand \hbPhi{\hat{\mathbf{\Phi}}}
\newcommand \hbPsi{\hat{\mathbf{\Psi}}}
\newcommand \hbOmega{\hat{\mathbf{\Omega}}}

%% BAR-BOLD
\newcommand \bba{\bar{\mathbf{a}}}
\newcommand \bbb{\bar{\mathbf{b}}}
\newcommand \bbc{\bar{\mathbf{c}}}
\newcommand \bbd{\bar{\mathbf{d}}}
\newcommand \bbe{\bar{\mathbf{e}}}
\newcommand \bbf{\bar{\mathbf{f}}}
\newcommand \bbh{\bar{\mathbf{h}}}
\newcommand \bbi{\bar{\mathbf{i}}}
\newcommand \bbj{\bar{\mathbf{j}}}
\newcommand \bbk{\bar{\mathbf{k}}}
\newcommand \bbell{\bar{\mathbf{\ell}}}
\newcommand \bbm{\bar{\mathbf{m}}}
\newcommand \bbn{\bar{\mathbf{n}}}
\newcommand \bbo{\bar{\mathbf{o}}}
\newcommand \bbp{\bar{\mathbf{p}}}
\newcommand \bbq{\bar{\mathbf{q}}}
\newcommand \bbr{\bar{\mathbf{r}}}
\newcommand \bbs{\bar{\mathbf{s}}}
\newcommand \bbt{\bar{\mathbf{t}}}
\newcommand \bbu{\bar{\mathbf{u}}}
\newcommand \bbv{\bar{\mathbf{v}}}
\newcommand \bbw{\bar{\mathbf{w}}}
\newcommand \bbx{\bar{\mathbf{x}}}
\newcommand \bby{\bar{\mathbf{y}}}
\newcommand \bbz{\bar{\mathbf{z}}}
\newcommand \bbA{\bar{\mathbf{A}}}
\newcommand \bbB{\bar{\mathbf{B}}}
\newcommand \bbC{\bar{\mathbf{C}}}
\newcommand \bbD{\bar{\mathbf{D}}}
\newcommand \bbE{\bar{\mathbf{E}}}
\newcommand \bbF{\bar{\mathbf{F}}}
\newcommand \bbG{\bar{\mathbf{G}}}
\newcommand \bbH{\bar{\mathbf{H}}}
\newcommand \bbI{\bar{\mathbf{I}}}
\newcommand \bbJ{\bar{\mathbf{J}}}
\newcommand \bbK{\bar{\mathbf{K}}}
\newcommand \bbL{\bar{\mathbf{L}}}
\newcommand \bbM{\bar{\mathbf{M}}}
\newcommand \bbN{\bar{\mathbf{N}}}
\newcommand \bbO{\bar{\mathbf{O}}}
\newcommand \bbP{\bar{\mathbf{P}}}
\newcommand \bbQ{\bar{\mathbf{Q}}}
\newcommand \bbR{\bar{\mathbf{R}}}
\newcommand \bbS{\bar{\mathbf{S}}}
\newcommand \bbT{\bar{\mathbf{T}}}
\newcommand \bbU{\bar{\mathbf{U}}}
\newcommand \bbV{\bar{\mathbf{V}}}
\newcommand \bbW{\bar{\mathbf{W}}}
\newcommand \bbX{\bar{\mathbf{X}}}
\newcommand \bbY{\bar{\mathbf{Y}}}
\newcommand \bbZ{\bar{\mathbf{Z}}}
\newcommand \bbalpha{\bar{\boldsymbol{\alpha}}}
\newcommand \bbbeta{\bar{\boldsymbol{\beta}}}
\newcommand \bbgamma{\bar{\boldsymbol{\gamma}}}
\newcommand \bbdelta{\bar{\boldsymbol{\delta}}}
\newcommand \bbepsilon{\bar{\boldsymbol{\epsilon}}}
\newcommand \bbzeta{\bar{\boldsymbol{\zeta}}}
\newcommand \bbtheta{\bar{\boldsymbol{\theta}}}
\newcommand \bbiota{\bar{\boldsymbol{\iota}}}
\newcommand \bbkappa{\bar{\boldsymbol{\kappa}}}
\newcommand \bblambda{\bar{\boldsymbol{\lambda}}}
\newcommand \bbmu{\bar{\boldsymbol{\mu}}}
\newcommand \bbnu{\bar{\boldsymbol{\nu}}}
\newcommand \bbxi{\bar{\boldsymbol{\xi}}}
\newcommand \bbpi{\bar{\boldsymbol{\pi}}}
\newcommand \bbrho{\bar{\boldsymbol{\rho}}}
\newcommand \bbsigma{\bar{\boldsymbol{\sigma}}}
\newcommand \bbtau{\bar{\boldsymbol{\tau}}}
\newcommand \bbupsilon{\bar{\boldsymbol{\upsilon}}}
\newcommand \bbphi{\bar{\boldsymbol{\phi}}}
\newcommand \bbchi{\bar{\boldsymbol{\chi}}}
\newcommand \bbpsi{\bar{\boldsymbol{\psi}}}
\newcommand \bbomega{\bar{\boldsymbol{\omega}}}
\newcommand \bbGamma{\bar{\mathbf{\Gamma}}}
\newcommand \bbDelta{\bar{\mathbf{\Delta}}}
\newcommand \bbTheta{\bar{\mathbf{\Theta}}}
\newcommand \bbLambda{\bar{\mathbf{\Lambda}}}
\newcommand \bbXi{\bar{\mathbf{\Xi}}}
\newcommand \bbPi{\bar{\mathbf{\Pi}}}
\newcommand \bbSigma{\bar{\mathbf{\Sigma}}}
\newcommand \bbPhi{\bar{\mathbf{\Phi}}}
\newcommand \bbPsi{\bar{\mathbf{\Psi}}}
\newcommand \bbOmega{\bar{\mathbf{\Omega}}}

%%%%%%%%%%%%%%%%DOT_BOLD
\newcommand \bdk{\dot{\mathbf{k}}}
\newcommand \bdK{\dot{\mathbf{K}}}

\newcommand \bdy{\dot{\mathbf{y}}}
\newcommand \bdY{\dot{\mathbf{Y}}}


%%%%%%%%%%%%%%%% HAT_DOT_BOLD
\newcommand \hbdy{\hat{\dot{\mathbf{y}}}}
\newcommand \hbdY{\hat{\dot{\mathbf{Y}}}}
